Sensitivity to light sterile neutrino mixing parameters with KM3NeT/ORCA

KM3NeT/ORCA is a next-generation neutrino telescope optimised for atmospheric neutrino oscillations studies. In this paper, the sensitivity of ORCA to the presence of a light sterile neutrino in a 3+1 model is presented. After three years of data taking, ORCA will be able to probe the active-sterile mixing angles $\theta_{14}$, $\theta_{24}$, $\theta_{34}$ and the effective angle $\theta_{\mu e}$, over a broad range of mass squared difference $\Delta m^2_{41} \sim [10^{-5}, 10]$ $\rm{eV}^2$, allowing to test the eV-mass sterile neutrino hypothesis as the origin of short baseline anomalies, as well as probing the hypothesis of a very light sterile neutrino, not yet constrained by cosmology. ORCA will be able to explore a relevant fraction of the parameter space not yet reached by present measurements.

==> authorlist.tex <==


%% The amssymb package provides various useful mathematical symbols
%\usepackage{amssymb}
%\usepackage{amsmath}
%\usepackage{subcaption}


%% The amsthm package provides extended theorem environments
%% \usepackage{amsthm}


%\journal{}


%\begin{frontmatter}

%% Title, authors and addresses

%% use the tnoteref command within \title for footnotes;
%% use the tnotetext command for theassociated footnote;
%% use the fnref command within \author or \affiliation for footnotes;
%% use the fntext command for theassociated footnote;
%% use the corref command within \author for corresponding author footnotes;
%% use the cortext command for theassociated footnote;
%% use the ead command for the email address,
%% and the form \ead[url] for the home page:
%% \title{Title\tnoteref{label1}}
%% \tnotetext[label1]{}
%% \author{Name\corref{cor1}\fnref{label2}}
%% \ead{email address}
%% \ead[url]{home page}
%% \fntext[label2]{}
%% \cortext[cor1]{}
%% \affiliation{Address\fnref{label3}}
%% \fntext[label3]{}

%\title{Sensitivity to light Sterile Neutrino Mixing Parameters with KM3NeT/ORCA}

%% use optional labels to link authors explicitly to addresses:

% ----- Start automatically generated KM3NeT info
% ----- Start author list

%\cortext[cor]{corresponding author}

\author[a]{S.~Aiello}
\author[bc,b]{A.~Albert}
\author[c]{M.~Alshamsi}
\author[d]{S. Alves Garre}
\author[e]{Z.~Aly}
\author[f,g]{A. Ambrosone}
\author[h]{F.~Ameli}
\author[i]{M.~Andre}
\author[j]{G.~Androulakis}
\author[k]{M.~Anghinolfi}
\author[l]{M.~Anguita}
\author[m]{G.~Anton}
\author[n]{M. Ardid}
\author[n]{S. Ardid}
\author[c]{J.~Aublin}
\author[j]{C.~Bagatelas}
\author[c]{B.~Baret}
\author[o]{S.~Basegmez~du~Pree}
\author[c,p]{M.~Bendahman}
\author[q,r]{F.~Benfenati}
\author[o]{E.~Berbee}
\author[s]{A.\,M.~van~den~Berg}
\author[e]{V.~Bertin}
\author[t]{S.~Biagi}
\author[m]{M.~Bissinger}
\author[u]{M.~Boettcher}
\author[v]{M.~Bou~Cabo}
\author[p]{J.~Boumaaza}
\author[w]{M.~Bouta}
\author[o]{M.~Bouwhuis}
\author[x]{C.~Bozza}
\author[y]{H.Br\^{a}nza\c{s}}
\author[z]{F.~Bretaudeau}
\author[o,aa]{R.~Bruijn}
\author[e]{J.~Brunner}
\author[a]{R.~Bruno}
\author[ab]{E.~Buis}
\author[f,ac]{R.~Buompane}
\author[e]{J.~Busto}
\author[k]{B.~Caiffi}
\author[d]{D.~Calvo}
\author[ad]{S.~Campion}
\author[ae,h]{A.~Capone}
\author[d]{V.~Carretero}
\author[q,af]{P.~Castaldi}
\author[ae,h]{S.~Celli}
\author[ag]{M.~Chabab}
\author[c]{N.~Chau}
\author[ah]{A.~Chen}
\author[t,ai]{S.~Cherubini}
\author[aj]{V.~Chiarella}
\author[q]{T.~Chiarusi}
\author[ak]{M.~Circella}
\author[t]{R.~Cocimano}
\author[c]{J.\,A.\,B.~Coelho}%\corref{cor}}

\author[c]{A.~Coleiro}
\author[c,d]{M.~Colomer~Molla}
\author[t]{R.~Coniglione}
\author[e]{P.~Coyle}
\author[c]{A.~Creusot}
\author[al]{A.~Cruz}
\author[t]{G.~Cuttone}
\author[z]{R.~Dallier}
\author[e]{B.~De~Martino}
\author[ak,am]{M.~De~Palma}
\author[ae,h]{I.~Di~Palma}
\author[l]{A.\,F.~D\'\i{}az}
\author[n]{D.~Diego-Tortosa}
\author[t]{C.~Distefano}
\author[k,an]{A.~Domi}%\corref{cor}}

\author[c]{C.~Donzaud}
\author[e]{D.~Dornic}
\author[ao]{M.~D{\"o}rr}
\author[bc,b]{D.~Drouhin}
\author[m]{T.~Eberl}
\author[p]{A.~Eddyamoui}
\author[o]{T.~van~Eeden}
\author[o]{D.~van~Eijk}
\author[w]{I.~El~Bojaddaini}
\author[ao]{D.~Elsaesser}
\author[e]{A.~Enzenh\"ofer}
\author[n]{V. Espinosa}
\author[ae,h]{P.~Fermani}
\author[t,ai]{G.~Ferrara}
\author[ap]{M.~D.~Filipovi\'c}
\author[q,r]{F.~Filippini}
\author[e]{L.\,A.~Fusco}
\author[m]{T.~Gal}
\author[n]{J.~Garc{\'\i}a~M{\'e}ndez}
\author[o]{A.~Garcia~Soto}
\author[f,g]{F.~Garufi}
\author[c]{Y.~Gatelet}
\author[m]{N.~Gei{\ss}elbrecht}
\author[f,ac]{L.~Gialanella}
\author[t]{E.~Giorgio}
\author[h,ad]{S.\,R.~Gozzini}
\author[o]{R.~Gracia}
\author[m]{K.~Graf}
\author[aq]{G.~Grella}
\author[bd]{D.~Guderian}
\author[k,an]{C.~Guidi}
\author[ar]{M.~Guti{\'e}rrez}
\author[m]{J.~Haefner}
\author[m]{S.~Hallmann}
\author[p]{H.~Hamdaoui}
\author[as]{H.~van~Haren}
\author[o]{A.~Heijboer}
\author[ao]{A.~Hekalo}
\author[m]{L.~Hennig}
\author[d]{J.\,J.~Hern{\'a}ndez-Rey}
\author[m]{J.~Hofest\"adt}
\author[e]{F.~Huang}
\author[f,ac]{W.~Idrissi~Ibnsalih}
\author[q,c]{G.~Illuminati}
\author[al]{C.\,W.~James}
\author[o]{M.~de~Jong}
\author[o,aa]{P.~de~Jong}
\author[o]{B.\,J.~Jung}
\author[ao]{M.~Kadler}
\author[at]{P.~Kalaczy\'nski}
\author[m]{O.~Kalekin}
\author[m]{U.\,F.~Katz}
\author[d]{N.\,R.~Khan~Chowdhury}
\author[au]{G.~Kistauri}
\author[ab]{F.~van~der~Knaap}
\author[aa,be]{P.~Kooijman}
\author[c,av]{A.~Kouchner}
\author[k]{V.~Kulikovskiy}
\author[m]{R.~Lahmann}
\author[c]{M.~Lamoureux}
\author[v]{G.~Lara}
\author[t]{G.~Larosa}
\author[e]{C.~Lastoria}
\author[c]{R.~Le~Breton}
\author[e]{S.~Le~Stum}
\author[t]{O.~Leonardi}
\author[t,ai]{F.~Leone}
\author[a]{E.~Leonora}
\author[m]{N.~Lessing}
\author[q,r]{G.~Levi}
\author[e]{M.~Lincetto}
\author[c]{M.~Lindsey~Clark}
\author[z]{T.~Lipreau}
\author[a]{F.~Longhitano}
\author[ar]{D.~Lopez-Coto}
\author[j]{A.~Lygda}
\author[c]{L.~Maderer}
\author[d]{J.~Ma\'nczak}
\author[ao]{K.~Mannheim}
\author[q,r]{A.~Margiotta}
\author[f]{A.~Marinelli}
\author[j]{C.~Markou}
\author[z]{L.~Martin}
\author[n]{J.\,A.~Mart{\'\i}nez-Mora}
\author[aj]{A.~Martini}
\author[f,ac]{F.~Marzaioli}
\author[f]{S.~Mastroianni}
\author[o]{K.\,W.~Melis}
\author[f,g]{G.~Miele}
\author[f]{P.~Migliozzi}
\author[t]{E.~Migneco}
\author[at]{P.~Mijakowski}
\author[aw]{L.\,S.~Miranda}
\author[f]{C.\,M.~Mollo}
\author[m]{M.~Moser}
\author[w]{A.~Moussa}
\author[o]{R.~Muller}
\author[t]{M.~Musumeci}
\author[o]{L.~Nauta}
\author[ar]{S.~Navas}
\author[h]{C.\,A.~Nicolau}
\author[ah]{B.~Nkosi}
\author[o,aa]{B.~{\'O}~Fearraigh}
\author[al]{M.~O'Sullivan}
\author[b]{M.~Organokov}
\author[t]{A.~Orlando}
\author[d]{J.~Palacios~Gonz{\'a}lez}
\author[au]{G.~Papalashvili}
\author[t]{R.~Papaleo}
\author[ak]{C.~Pastore}
\author[y]{A.~M.~P{\u a}un}
\author[y]{G.\,E.~P\u{a}v\u{a}la\c{s}}
\author[r,bf]{C.~Pellegrino}
\author[e]{S. Pe\~{n}a Mart\'inez}
\author[e]{M.~Perrin-Terrin}
\author[o]{V.~Pestel}
\author[t]{P.~Piattelli}
\author[d]{C.~Pieterse}
\author[f,g]{O.~Pisanti}
\author[n]{C.~Poir{\`e}}
\author[f]{V.~Pontoriere}
\author[y]{V.~Popa}
\author[b]{T.~Pradier}
\author[m]{I.~Probst}
\author[ax]{G.~P{\"u}hlhofer}
\author[t]{S.~Pulvirenti}
\author[a]{N.~Randazzo}
\author[aw]{S.~Razzaque}
\author[d]{D.~Real}
\author[m]{S.~Reck}
\author[t]{G.~Riccobene}
\author[k,an]{A.~Romanov}
\author[t]{A.~Rovelli}
\author[d]{F.~Salesa~Greus}
\author[o,ay]{D.\,F.\,E.~Samtleben}
\author[ak]{A.~S{\'a}nchez~Losa}
\author[k,an]{M.~Sanguineti}
\author[ax]{A.~Santangelo}
\author[t]{D.~Santonocito}
\author[t]{P.~Sapienza}
\author[m]{J.~Schnabel}
\author[m]{M.\,F.~Schneider}
\author[m]{J.~Schumann}
\author[u]{H.~M. Schutte}
\author[o]{J.~Seneca}
\author[ak]{I.~Sgura}
\author[au]{R.~Shanidze}
\author[az]{A.~Sharma}
\author[j]{A.~Sinopoulou}
\author[aq,f]{B.~Spisso}
\author[q,r]{M.~Spurio}
\author[j]{D.~Stavropoulos}
\author[aq,f]{S.\,M.~Stellacci}
\author[k,an]{M.~Taiuti}
\author[ak]{F.~Tatone}
\author[p]{Y.~Tayalati}
\author[d]{T.~Thakore}%\corref{cor}}

\author[u]{H.~Thiersen}
\author[al]{S.~Tingay}
\author[j]{S.~Tsagkli}
\author[j]{V.~Tsourapis}
\author[j]{E.~Tzamariudaki}
\author[j]{D.~Tzanetatos}
\author[c,av]{V.~Van~Elewyck}
\author[ba]{G.~Vasileiadis}
\author[q,r]{F.~Versari}
\author[f,ac]{D.~Vivolo}
\author[c]{G.~de~Wasseige}
\author[bb]{J.~Wilms}
\author[at]{R.~Wojaczy\'nski}
\author[o,aa]{E.~de~Wolf}
\author[w]{T.~Yousfi}
\author[k]{S.~Zavatarelli}
\author[ae,h]{A.~Zegarelli}
\author[t]{D.~Zito}
\author[d]{J.\,D.~Zornoza}
\author[d]{J.~Z{\'u}{\~n}iga}
\author[u]{N.~Zywucka}
% ----- End author list
% ----- Start affiliation list
\affiliation[a]{INFN, Sezione di Catania, Via Santa Sofia 64, Catania, 95123 Italy}
\affiliation[b]{Universit{\'e}~de~Strasbourg,~CNRS,~IPHC~UMR~7178,~F-67000~Strasbourg,~France}
\affiliation[c]{Universit{\'e} de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\affiliation[d]{IFIC - Instituto de F{\'\i}sica Corpuscular (CSIC - Universitat de Val{\`e}ncia), c/Catedr{\'a}tico Jos{\'e} Beltr{\'a}n, 2, 46980 Paterna, Valencia, Spain}
\affiliation[e]{Aix~Marseille~Univ,~CNRS/IN2P3,~CPPM,~Marseille,~France}
\affiliation[f]{INFN, Sezione di Napoli, Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\affiliation[g]{Universit{\`a} di Napoli ``Federico II'', Dip. Scienze Fisiche ``E. Pancini'', Complesso Universitario di Monte S. Angelo, Via Cintia ed. G, Napoli, 80126 Italy}
\affiliation[h]{INFN, Sezione di Roma, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation[i]{Universitat Polit{\`e}cnica de Catalunya, Laboratori d'Aplicacions Bioac{\'u}stiques, Centre Tecnol{\`o}gic de Vilanova i la Geltr{\'u}, Avda. Rambla Exposici{\'o}, s/n, Vilanova i la Geltr{\'u}, 08800 Spain}
\affiliation[j]{NCSR Demokritos, Institute of Nuclear and Particle Physics, Ag. Paraskevi Attikis, Athens, 15310 Greece}
\affiliation[k]{INFN, Sezione di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation[l]{University of Granada, Dept.~of Computer Architecture and Technology/CITIC, 18071 Granada, Spain}
\affiliation[m]{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, Erlangen Centre for Astroparticle Physics, Erwin-Rommel-Stra{\ss}e 1, 91058 Erlangen, Germany}
\affiliation[n]{Universitat Polit{\`e}cnica de Val{\`e}ncia, Instituto de Investigaci{\'o}n para la Gesti{\'o}n Integrada de las Zonas Costeras, C/ Paranimf, 1, Gandia, 46730 Spain}
\affiliation[o]{Nikhef, National Institute for Subatomic Physics, PO Box 41882, Amsterdam, 1009 DB Netherlands}
\affiliation[p]{University Mohammed V in Rabat, Faculty of Sciences, 4 av.~Ibn Battouta, B.P.~1014, R.P.~10000 Rabat, Morocco}
\affiliation[q]{INFN, Sezione di Bologna, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\affiliation[r]{Universit{\`a} di Bologna, Dipartimento di Fisica e Astronomia, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
\affiliation[s]{KVI-CART~University~of~Groningen,~Groningen,~the~Netherlands}
\affiliation[t]{INFN, Laboratori Nazionali del Sud, Via S. Sofia 62, Catania, 95123 Italy}
\affiliation[u]{North-West University, Centre for Space Research, Private Bag X6001, Potchefstroom, 2520 South Africa}
\affiliation[v]{Instituto Espa{\~n}ol de Oceanograf{\'\i}a, Unidad Mixta IEO-UPV, C/ Paranimf, 1, Gandia, 46730 Spain}
\affiliation[w]{University Mohammed I, Faculty of Sciences, BV Mohammed VI, B.P.~717, R.P.~60000 Oujda, Morocco}
\affiliation[x]{Universit{\`a} di Salerno e INFN Gruppo Collegato di Salerno, Dipartimento di Matematica, Via Giovanni Paolo II 132, Fisciano, 84084 Italy}
\affiliation[y]{ISS, Atomistilor 409, M\u{a}gurele, RO-077125 Romania}
\affiliation[z]{Subatech, IMT Atlantique, IN2P3-CNRS, Universit{\'e} de Nantes, 4 rue Alfred Kastler - La Chantrerie, Nantes, BP 20722 44307 France}
\affiliation[aa]{University of Amsterdam, Institute of Physics/IHEF, PO Box 94216, Amsterdam, 1090 GE Netherlands}
\affiliation[ab]{TNO, Technical Sciences, PO Box 155, Delft, 2600 AD Netherlands}
\affiliation[ac]{Universit{\`a} degli Studi della Campania "Luigi Vanvitelli", Dipartimento di Matematica e Fisica, viale Lincoln 5, Caserta, 81100 Italy}
\affiliation[ad]{University La Sapienza, Roma, Physics Department, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation[ae]{Universit{\`a} La Sapienza, Dipartimento di Fisica, Piazzale Aldo Moro 2, Roma, 00185 Italy}
\affiliation[af]{Universit{\`a} di Bologna, Dipartimento di Ingegneria dell'Energia Elettrica e dell'Informazione "Guglielmo Marconi", Via dell'Universit{\`a} 50, Cesena, 47521 Italia}
\affiliation[ag]{Cadi Ayyad University, Physics Department, Faculty of Science Semlalia, Av. My Abdellah, P.O.B. 2390, Marrakech, 40000 Morocco}
\affiliation[ah]{University of the Witwatersrand, School of Physics, Private Bag 3, Johannesburg, Wits 2050 South Africa}
\affiliation[ai]{Universit{\`a} di Catania, Dipartimento di Fisica e Astronomia "Ettore Majorana", Via Santa Sofia 64, Catania, 95123 Italy}
\affiliation[aj]{INFN, LNF, Via Enrico Fermi, 40, Frascati, 00044 Italy}
\affiliation[ak]{INFN, Sezione di Bari, via Orabona, 4, Bari, 70125 Italy}
\affiliation[al]{International Centre for Radio Astronomy Research, Curtin University, Bentley, WA 6102, Australia}
\affiliation[am]{University of Bari, Via Amendola 173, Bari, 70126 Italy}
\affiliation[an]{Universit{\`a} di Genova, Via Dodecaneso 33, Genova, 16146 Italy}
\affiliation[ao]{University W{\"u}rzburg, Emil-Fischer-Stra{\ss}e 31, W{\"u}rzburg, 97074 Germany}
\affiliation[ap]{Western Sydney University, School of Computing, Engineering and Mathematics, Locked Bag 1797, Penrith, NSW 2751 Australia}
\affiliation[aq]{Universit{\`a} di Salerno e INFN Gruppo Collegato di Salerno, Dipartimento di Fisica, Via Giovanni Paolo II 132, Fisciano, 84084 Italy}
\affiliation[ar]{University of Granada, Dpto.~de F\'\i{}sica Te\'orica y del Cosmos \& C.A.F.P.E., 18071 Granada, Spain}
\affiliation[as]{NIOZ (Royal Netherlands Institute for Sea Research), PO Box 59, Den Burg, Texel, 1790 AB, the Netherlands}
\affiliation[at]{National~Centre~for~Nuclear~Research,~02-093~Warsaw,~Poland}
\affiliation[au]{Tbilisi State University, Department of Physics, 3, Chavchavadze Ave., Tbilisi, 0179 Georgia}
\affiliation[av]{Institut Universitaire de France, 1 rue Descartes, Paris, 75005 France}
\affiliation[aw]{University of Johannesburg, Department Physics, PO Box 524, Auckland Park, 2006 South Africa}
\affiliation[ax]{Eberhard Karls Universit{\"a}t T{\"u}bingen, Institut f{\"u}r Astronomie und Astrophysik, Sand 1, T{\"u}bingen, 72076 Germany}
\affiliation[ay]{Leiden University, Leiden Institute of Physics, PO Box 9504, Leiden, 2300 RA Netherlands}
\affiliation[az]{Universit{\`a} di Pisa, Dipartimento di Fisica, Largo Bruno Pontecorvo 3, Pisa, 56127 Italy}
\affiliation[ba]{Laboratoire Univers et Particules de Montpellier, Place Eug{\`e}ne Bataillon - CC 72, Montpellier C{\'e}dex 05, 34095 France}
\affiliation[bb]{Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, Remeis Sternwarte, Sternwartstra{\ss}e 7, 96049 Bamberg, Germany}
\affiliation[bc]{Universit{\'e} de Strasbourg, Universit{\'e} de Haute Alsace, GRPHE, 34, Rue du Grillenbreit, Colmar, 68008 France}
\affiliation[bd]{University of M{\"u}nster, Institut f{\"u}r Kernphysik, Wilhelm-Klemm-Str. 9, M{\"u}nster, 48149 Germany}
\affiliation[be]{Utrecht University, Department of Physics and Astronomy, PO Box 80000, Utrecht, 3508 TA Netherlands}
\affiliation[bf]{INFN, CNAF, v.le C. Berti-Pichat, 6/2, Bologna, 40127 Italy}
% ----- End affiliation list
% ----- End automatically generated KM3NeT info


%\end{frontmatter}

%%\linenumbers

%% main text

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput
%%
%% End of file `elsarticle-template-num.tex'.

